Physics-guided Terahertz Computational Imaging

Visualizing information inside objects is an ever-lasting need to bridge the world from physics, chemistry, biology to computation. Among all tomographic techniques, terahertz (THz) computational imaging has demonstrated its unique sensing features to digitalize multi-dimensional object information in a non-destructive, non-ionizing, and non-invasive way. Applying modern signal processing and physics-guided modalities, THz computational imaging systems are now launched in various application fields in industrial inspection, security screening, chemical inspection and non-destructive evaluation. In this article, we overview recent advances in THz computational imaging modalities in the aspects of system configuration, wave propagation and interaction models, physics-guided algorithm for digitalizing interior information of imaged objects. Several image restoration and reconstruction issues based on multi-dimensional THz signals are further discussed, which provides a crosslink between material digitalization, functional property extraction, and multi-dimensional imager utilization from a signal processing perspective.

==> Acknowledgement.tex <==
This work was financially supported in part from the Young Scholar Fellowship Program  under Grant MOST 110-2636-E-007-017, and in part from the AI Innovation Research Program under Grant MOST 110-2634-F-007-015, by Ministry of Science and Technology (MOST) in Taiwan.

==> README <==

August 26, 2015


IEEEtran is a LaTeX class for authors of the Institute of Electrical and
Electronics Engineers (IEEE) transactions journals and conferences.
The latest version of the IEEEtran package can be found at CTAN:

http://www.ctan.org/pkg/ieeetran

as well as within IEEE's site:

http://www.ieee.org/

For latest news, helpful tips, answers to frequently asked questions,
beta releases and other support, visit the IEEEtran home page at my
website:

http://www.michaelshell.org/tex/ieeetran/

Version 1.8b has a number of significant changes over the v1.8a release.
For a full history of changes, please read the file changelog.txt.
The most notable changes in this release include:

 1) Added new comsoc mode for the IEEE Communications Society.
    This mode (at present) only invokes the use of the newtxmath math fonts.
 
 2) Revised IEEEeqnarray column specifications to work with active " 
    (or other punctuation catcode changes) as with babel under the
    german or ngerman language modes. 
    Thanks to Stefan M. Moser for reporting this problem.

 3) Added \indexspace and other index related macros as newer versions of
    article.cls now do. These macros are needed to avoid an error when
    using the glossaries package.
    Thanks to Sebastian Nyberg for suggesting this change.

 4) Fixed odd/even page header font bug under compsoc mode and
    other page style code improvements.
    Thanks to Marco Paolieri for reporting this problem.

 5) Added hooks to allow for easy control of spacing above title.

 6) Added the \IEEEnoauxwrite command.
    Thanks to Sudarshan Mukherjee for suggesting this feature.


NOTE: Take care not to confuse the "comsoc" and "compsoc" class
options/modes as they are very different:

comsoc  ==> IEEE Communications Society
compsoc ==> IEEE Computer Society

The comsoc mode requires that an acceptable Times math font be available on
the LaTeX system. This requirement will be enforced by IEEEtran in comsoc
mode. Either the freely available newtxmath font by Michael Sharpe
http://www.ctan.org/pkg/newtx
(version 1.451, July 28, 2015 or later is recommended)
or the commercial MathTime font (e.g., mtpro2.sty) is acceptable.
See Section II-D (2.4) "Class Options - comsoc, compsoc, transmag" of
the IEEEtran HOWTO for more details.


Best wishes for all your publication endeavors,

Michael Shell
http://www.michaelshell.org/


********************************** Files **********************************

README                 - This file.

IEEEtran.cls           - The IEEEtran LaTeX class file.

changelog.txt          - The revision history.

IEEEtran_HOWTO.pdf     - The IEEEtran LaTeX class user manual.

bare_conf.tex          - A bare bones starter file for IEEE conference papers.

bare_conf_compsoc.tex  - A bare bones starter file for IEEE Computer Society
                         conference papers.

bare_jrnl.tex          - A bare bones starter file for IEEE journal papers.

bare_jrnl_comsoc.tex   - A bare bones starter file for IEEE Communications
                         Society journal papers.

bare_jrnl_compsoc.tex  - A bare bones starter file for IEEE Computer Society
                         journal papers.

bare_jrnl_transmag.tex - A bare bones starter file for IEEE Transactions
                         on Magnetics journal papers.

bare_adv.tex           - A bare bones starter file showing advanced
                         techniques such as conditional compilation,
                         hyperlinks, PDF thumbnails, etc. The illustrated
                         format is for an IEEE Computer Society journal paper.

***************************************************************************
Legal Notice:
This code is offered as-is without any warranty either expressed or
implied; without even the implied warranty of MERCHANTABILITY or
FITNESS FOR A PARTICULAR PURPOSE! 
User assumes all risk.
In no event shall the IEEE or any contributor to this code be liable for
any damages or losses, including, but not limited to, incidental,
consequential, or any other damages, resulting from the use or misuse
of any information contained here.

All comments are the opinions of their respective authors and are not
necessarily endorsed by the IEEE.

This work is distributed under the LaTeX Project Public License (LPPL)
( http://www.latex-project.org/ ) version 1.3, and may be freely used,
distributed and modified. A copy of the LPPL, version 1.3, is included
in the base LaTeX documentation of all distributions of LaTeX released
2003/12/01 or later.
Retain all contribution notices and credits.
** Modified files should be clearly indicated as such, including  **
** renaming them and changing author support contact information. **

File list of work: IEEEtran.cls, IEEEtran_HOWTO.pdf, bare_adv.tex,
                   bare_conf.tex, bare_conf_compsoc.tex, bare_jrnl.tex,
                   bare_jrnl_comsoc.tex, bare_jrnl_compsoc.tex,
                   bare_jrnl_transmag.tex
***************************************************************************


==> author.tex <==
\subsection{Ta-Hsuan Chao}
Ta-Hsuan Chao received his B.S. degree in electrical engineering in National Tsing Hua University, and he is the research assistant in the research group led by Shang-Hua Yang from National Tsing Hua University.

\subsection{Weng-Tai Su} 
Weng-Tai Su received the B.S. degree in electrical engineering from the National Yunlin University of Science and Technology, Yunlin, Taiwan, in 2012, and the M.S. degree in electrical engineering from the National Tsing Hua University, Hsinchu, Taiwan, in 2014. He is currently working toward the Ph.D. degree with the Department of Electrical Engineering, National Tsing Hua University. His research interests mainly include deep learning, graph signal processing, image/video processing, and image classification/clustering.

\subsection{Yi-Chun Hung}
XXX

\subsection{Che-Min Wu}
XXX


\subsection{Chia-Wen Lin} 
	(Fellow, IEEE) received his Ph.D. degree from National Tsing Hua University (NTHU), Taiwan, in 2000.  
	Dr. Lin is currently Professor with the Department of Electrical Engineering and the Institute of Communications Engineering, NTHU.   His research interests include image and video processing, computer vision, and video networking.  He served as Distinguished Lecturer of IEEE Circuits and Systems Society (2018--2019). He has served on the editorial boards of TMM, TIP, TCSVT, IEEE Multimedia, and Elsevier JVCI.  He is Chair of ICME Steering Committee and was Steering Committee member of IEEE TMM from 2013 to 2015. He served as TPC Co-Chair of ICIP 2019 and ICME 2010, and General Co-Chair of VCIP 2018. He received best paper awards from VCIP 2010 and 2015.
	
\subsection{Shang-Hua Yang} 
	(Member, IEEE) is a tenure-track assistant professor in the Department of Electrical Engineering at National Tsing Hua University (NTHU). He received his Ph.D. degree in electrical engineering from the University of Michigan Ann Arbor in 2016. Dr. Yang has established contributions to the development of ultrafast electronics, microwave photonics, terahertz optoelectronics, integrated terahertz systems as well as plasmonic photonics applications. The outcomes of his research have appeared in over 70 refereed papers in peer-reviewed journals and conference proceedings on these topics. He has received several prestigious awards and scholarships including, SPIE Scholarship in Optics and photonics (2012), IEEE Antennas and Propagation Society Doctoral Research Award (2014),  Joan and Irvin Jacobs TIX Institute Industry Scholar (2017, 2018), MOST Young Scholar Fellowship (2018) and Human Frontier Science Program Research Grant Award (2020). Dr. Yang is currently the co-founder and deputy director of NTHU Terahertz Optics \& Photonics Center (2019 - present).	


==> bio.tex <==
\vspace{0.1in}


% \begin{IEEEbiography}[{\includegraphics[width=1in,height=1.1in,clip,keepaspectratio]{fig/thchao.jpg}}]{Ta-Hsuan Chao}

%     Ta-Hsuan Chao received his B.S. degree in electrical engineering in National Tsing Hua University, and he is the research assistant in the research group led by Shang-Hua Yang from National Tsing Hua University.
    
%     His research interests are natural language processing, computer vision, machine learning, and terahertz imaging.
    
% \end{IEEEbiography}
% \vspace{-0.2 in}

% \begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{fig/wtsu.jpg}}]{Weng-Tai Su}
		
% 	Weng-Tai Su received the B.S. degree in electrical engineering from the National Yunlin University of Science and Technology, Yunlin, Taiwan, in 2012, Taiwan, the M.S. degree in electrical engineering from National Tsing Hua University (NTHU), Hsinchu, Taiwan, in 2014. He is currently pursuing his Ph.D. degree at the Department of Electrical Engineering of NTHU.
	
% 	His research interests mainly lie in machine learning, image and video processing, and computer vision. 
% \end{IEEEbiography}

% \vspace{-0.2in}

% \begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{fig/wtsu.jpg}}]{Yi-Chun Hung}
		
% 	XXX
	
% \end{IEEEbiography}

% \vspace{-0.2in}

% \begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{fig/wtsu.jpg}}]{Che-Min Wu}
		
% 	XXX
	
% \end{IEEEbiography}

% \vspace{-0.2in}

% \begin{IEEEbiography}
% 	[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio] {fig/cwlin.jpg}}]
% 	{Chia-Wen Lin}
% 	(Fellow, IEEE) received his Ph.D. degree from National Tsing Hua University (NTHU), Taiwan, in 2000.  
% 	Dr. Lin is currently Professor with the Department of Electrical Engineering and the Institute of Communications Engineering, NTHU.   His research interests include image and video processing, computer vision, and video networking.  He served as Distinguished Lecturer of IEEE Circuits and Systems Society (2018--2019). He has served on the editorial boards of TMM, TIP, TCSVT, IEEE Multimedia, and Elsevier JVCI.  He is Chair of ICME Steering Committee and was Steering Committee member of IEEE TMM from 2013 to 2015. He served as TPC Co-Chair of ICIP 2019 and ICME 2010, and General Co-Chair of VCIP 2018. He received best paper awards from VCIP 2010 and 2015.
% \end{IEEEbiography}

% \vspace{-0.2 in}

% \begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{fig/shyang.jpg}}]{Shang-Hua Yang}
	
% 	(Member, IEEE) is a tenure-track assistant professor in the Department of Electrical Engineering at National Tsing Hua University (NTHU). He received his Ph.D. degree in electrical engineering from the University of Michigan Ann Arbor in 2016. Dr. Yang has established contributions to the development of ultrafast electronics, microwave photonics, terahertz optoelectronics, integrated terahertz systems as well as plasmonic photonics applications. The outcomes of his research have appeared in over 70 refereed papers in peer-reviewed journals and conference proceedings on these topics. He has received several prestigious awards and scholarships including, SPIE Scholarship in Optics and photonics (2012), IEEE Antennas and Propagation Society Doctoral Research Award (2014),  Joan and Irvin Jacobs TIX Institute Industry Scholar (2017, 2018), MOST Young Scholar Fellowship (2018) and Human Frontier Science Program Research Grant Award (2020). Dr. Yang is currently the co-founder and deputy director of NTHU Terahertz Optics \& Photonics Center (2019 - present).
	
% \end{IEEEbiography}
\textbf{Ta-Hsuan Chao} received his B.S. degree in electrical engineering in National Tsing Hua University, and he is the research assistant in the research group led by Shang-Hua Yang from National Tsing Hua University.
    
His research interests are natural language processing, computer vision, machine learning, and terahertz imaging.


\vspace{0.1in}
\textbf{Weng-Tai Su} received the B.S. degree in electrical engineering from the National Yunlin University of Science and Technology, Yunlin, Taiwan, in 2012, Taiwan, the M.S. degree in electrical engineering from National Tsing Hua University (NTHU), Hsinchu, Taiwan, in 2014. He is currently pursuing his Ph.D. degree at the Department of Electrical Engineering of NTHU.
	
	His research interests mainly lie in machine learning, image and video processing, and computer vision. 
	
\vspace{0.1in}	
\textbf{Yi-Chun Hung}
    received his B.S. degree in electrical engineering from National Tsing Hua University in 2019, and he is currently a graduate student in University of California, Los Angeles. His research interests lie in computational imaging, computer vision and deep learning.

\vspace{0.1in}
\textbf{Che-Min Wu}
    received the B.S. degree in Interdisciplinary Program of Electrical Engineering and Computer Science from National Tsing Hua University (NTHU), Hsinchu, Taiwan in 2018. He directly pursue the Ph.D. degree at the Institute of Electronic Engineering of NTHU. His research interests mainly lie in Terahertz spectroscopy and Terahertz nanoimaging.

\vspace{0.1in}
\textbf{Chia-Wen Lin}
	(Fellow, IEEE) received his Ph.D. degree from National Tsing Hua University (NTHU), Taiwan, in 2000.  
	Dr. Lin is currently Professor with the Department of Electrical Engineering and the Institute of Communications Engineering, NTHU.   His research interests include image and video processing, computer vision, and video networking.  He served as Distinguished Lecturer of IEEE Circuits and Systems Society (2018--2019). He has served on the editorial boards of TMM, TIP, TCSVT, IEEE Multimedia, and Elsevier JVCI.  He is Chair of ICME Steering Committee and was Steering Committee member of IEEE TMM from 2013 to 2015. He served as TPC Co-Chair of ICIP 2019 and ICME 2010, and General Co-Chair of VCIP 2018. He received best paper awards from VCIP 2010 and 2015.
	
\vspace{0.1in}
\textbf{Shang-Hua Yang}
	(Member, IEEE) is a tenure-track assistant professor in the Department of Electrical Engineering at National Tsing Hua University (NTHU). He received his Ph.D. degree in electrical engineering from the University of Michigan Ann Arbor in 2016. Dr. Yang has established contributions to the development of ultrafast electronics, microwave photonics, terahertz optoelectronics, integrated terahertz systems as well as plasmonic photonics applications. The outcomes of his research have appeared in over 70 refereed papers in peer-reviewed journals and conference proceedings on these topics. He has received several prestigious awards and scholarships including, SPIE Scholarship in Optics and photonics (2012), IEEE Antennas and Propagation Society Doctoral Research Award (2014),  Joan and Irvin Jacobs TIX Institute Industry Scholar (2017, 2018), MOST Young Scholar Fellowship (2018) and Human Frontier Science Program Research Grant Award (2020). Dr. Yang is currently the co-founder and deputy director of NTHU Terahertz Optics \& Photonics Center (2019 - present).






	
	





==> remark.tex <==
In this article, we overview terahertz tomographic imaging on for advanced materials exploration from theory to applications. The terahertz tomographic imaging  is similar to traditional image processing for standard signals, however, its realization is completely different due to xxxxxxxxxxxxxx. Current methods have found several interesting applications. At the same time, the following
issues, both theoretical and practical aspects, are still open:
